Bandit Algorithms for Precision Medicine

The Oxford English Dictionary defines precision medicine as "medical care designed to optimize efficiency or therapeutic benefit for particular groups of patients, especially by using genetic or molecular profiling." It is not an entirely new idea: physicians from ancient times have recognized that medical treatment needs to consider individual variations in patient characteristics. However, the modern precision medicine movement has been enabled by a confluence of events: scientific advances in fields such as genetics and pharmacology, technological advances in mobile devices and wearable sensors, and methodological advances in computing and data sciences. This chapter is about bandit algorithms: an area of data science of special relevance to precision medicine. With their roots in the seminal work of Bellman, Robbins, Lai and others, bandit algorithms have come to occupy a central place in modern data science ( Lattimore and Szepesvari, 2020). Bandit algorithms can be used in any situation where treatment decisions need to be made to optimize some health outcome. Since precision medicine focuses on the use of patient characteristics to guide treatment, contextual bandit algorithms are especially useful since they are designed to take such information into account. The role of bandit algorithms in areas of precision medicine such as mobile health and digital phenotyping has been reviewed before (Tewari and Murphy, 2017; Rabbi et al., 2019). Since these reviews were published, bandit algorithms have continued to find uses in mobile health and several new topics have emerged in the research on bandit algorithms. This chapter is written for quantitative researchers in fields such as statistics, machine learning, and operations research who might be interested in knowing more about the algorithmic and mathematical details of bandit algorithms that have been used in mobile health.

==> pure_exploration.tex <==
\ambuj{one problem with this entire pure exploration literature is that it is entirely theoretical. do we know of a single instance where any of these ideas were used in a real clinical trial? i think actual randomized clinical trials just use uniform random allocation with sample size chosen according to power calculations. i am struggling a bit to add proper motivation for this section. the mice example we give below is too naive in my opinion.}



All the policies introduced in previous sections were designed to maximize the cumulative reward which involves a trade-off between exploration and exploitation. 
In this section, we discuss a different setting where the exploration cost is not a concern and the agent just wants to output a final recommendation for the best arm after an exploration phase. 
For example, suppose that scientists are trying to figure out the most effective drug dose by performing $T$ experiments on mice before human trials. The outcomes of the $T$ experiments for the mice are not the concern here. Instead the scientists just want to make sure they can find the most effective dose.
Problems of this type are called \emph{pure exploration problems}. 
Formally speaking, the agent pulls arms for $T$ rounds ($T$ is not necessarily known in advance) aiming at identifying an arm $B_T$ with the largest mean as quickly and accurately as possible.

Algorithms for pure exploration problems are usually made of three components: 1) a sampling rule to determine $A_t$, the arm to explore at round $t$, 2) a recommendation rule $B_t$ which maintains the current guess for the best arm, and 3) a stopping rule $\tau$ which decides at which round we stop exploring and output the recommendation.
We summarize this procedure in Algorithm~\ref{algo:exploration}.
\begin{algorithm}[tbp]
	\caption{Pure Exploration Framework} 
	\begin{algorithmic}[1]
		\STATE \textbf{Input:} action set $\mathcal{A}$, a stopping rule $\tau$.
		\FOR{$t=1,2,3\ldots$}
		\STATE Sampling rule picks $A_t\in\mathcal{A}$. Obtain reward $R_t$.
		\STATE If stopping rule $\tau$ decides to stop, break.
		\ENDFOR
		\STATE \textbf{Output:} Let current time be $T$. Recommendation rule picks $B_T\in\mathcal{A}$.
	\end{algorithmic}
\label{algo:exploration}
\end{algorithm}
Pure exploration algorithms are evaluated using a performance measure called \emph{simple regret}. It is defined as the difference between the reward expectation of the optimal arm and the output arm:
\begin{align}
\text{Reg}_T^{\mathrm{Sim}}(\pi, \nu) = \mu^* - \mu_{B_T}.
\end{align}
We use $p_{\nu,\pi}(T)$ to denote the probability of error after $T$ rounds: $\mathbb{P}_{\nu, \pi}(B_{T}\neq a^*)$.
By definition, we see that $\Delta_{\mathrm{min}}p_{\nu,\pi}(T)\leq \mathbb{E}[R_T^{\mathrm{Sim}}(\pi, \nu)] \leq \Delta_{\mathrm{max}}p_{\nu,\pi}(T)$, where $\Delta_{\mathrm{min}}$ and $\Delta_{\mathrm{max}}$ represent the minimum/maximum gap between the optimal arm and other arms.
There are two major theoretical frameworks to study pure exploration problems: the \emph{fixed budget setting} and the \emph{fixed-confidence setting}. 
In the fixed-budget setting, the goal is to minimize $p_{\nu,\pi}(T)$ or $\mathbb{E}[R_T^{\mathrm{Sim}}(\pi,\nu)]$ within a fixed number of pulls $T$.
In the fixed-confidence setting, the goal is to minimize the number of pulls $\tau$ to guarantee $p_{\nu,\pi}(\tau)\leq \delta$ or $R_T^{\mathrm{Sim}}(\pi,\nu)$ is small with probability $1-\delta$.
We next introduce the results of several well-studied pure exploration algorithms for the MAB setting.

\subsubsection{Fixed-budget Setting}
A simple strategy for this setting is the uniform forecaster \ambuj{why "forecaster"? is this the standard name used in the literature?}, in which the agent pulls each arm one by one repeatedly for a total of $T$ rounds and recommends the arm with the highest empirical mean. 
\citet{bubeck2009pure} showed that the gap-dependent and worst-case expected simple regret for the uniform forecaster are $\sum_{j:\Delta_j>0}\Delta_j\exp\left(-T\Delta_j^2/2K\right)$ and $2\sqrt{2K\log K/T}$ respectively.
They also give a lower bound showing that $\mathbb{E}[R_T^{\mathrm{Sim}}(\pi,\nu)] = \Omega(\sqrt{K/T})$, which means that the uniform strategy is already tight up to logarithmic factors in $K$. 

Actually, any bandit algorithm $A_1$ with bounded cumulative regret can always be converted to its pure exploration variant $A_2$ by adding a recommendation rule in the end of $A_1$. Some natural recommendation rules are the empirically best arm, the most played arm, and sampling based on empirical distribution of plays.
For example, by running a UCB($p$) \ziping{It is better to remind the reader what $p$ represents here.} \ambuj{agreed} algorithm and recommending the arm with the highest empirical mean in the end, one can achieve $O(\sqrt{kp\log T/T})$ worst-case simple regret~\citep{bubeck2009pure}.
An interesting result shows that the cumulative regret upper bound for $A_1$ can be converted to a lower bound of the simple regret for $A_2$ and smaller cumulative regret can lead to larger simple regret. 
We refer the reader to \citet{bubeck2009pure} for more details on these relations. \ambuj{the beginning of this para suggests that it is about converting cumulative regret guarantees into simple regret. however, the last couple of sentences are pointing in the reverse direction. perhaps rewrite with a focus on what you want the reader to take away as the main message.}

Later on, \citet{audibert2010best} proposed the UCB exploration (UCB-E) algorithm by carefully tuning the exploration parameter using the reward gap information \ambuj{but reward gap info is not easily available. does the algo estimate it?}.
The algorithm satisfies $p_{\nu,\mathrm{UCB-E}}(T)\leq 2Tk\exp\left(-\frac{T-k}{18H_1}\right)$ where $H_1:=\sum_{i=1}^{k}\frac{1}{\Delta_i^2}$.
Action elimination based algorithms also work well. 
For example, the Successive Rejects~\citep{audibert2010best} and Sequential Halving~\citep{karnin2013almost} algorithms are both parameter-free and can guarantee identifying the best arm with high probability. \ambuj{are instance dependent lower bounds for pure exploration known?}

\subsubsection{Fixed-confidence Setting}
In this setting, the number of rounds is not fixed in advance. Instead, the agent decides a stopping rule based on the history. 
Several strategies have been proposed to minimize $\mathbb{E}_{\nu,\pi}[\tau]$ while ensuring that the best arm is identified with high probability.
In action elimination algorithms~\citep{even2002pac,karnin2013almost}, the agent maintains an action set $\Omega_t$, samples the arms in $\Omega_t$ for a predetermined number of times. 
The algorithm terminates when $|\Omega_t| = 1$ and outputs the single element in $\Omega_t$.
Another family of strategies uses upper and lower confidence bounds on the means of the arms to construct their sampling and stopping rules~\citep{audibert2010best,gabillon2012best,kalyanakrishnan2012pac,kaufmann2013information,jamieson2014lil}.
For example, the algorithm terminates when the lower confidence bound of one arm is already higher than the upper confidence bound of other arms.
Furthermore, \citet{garivier2016optimal} developed an asymptotically optimal strategy called ``Track-and-Stop" which combines a track of the optimal proportions for arm sampling with Chernoff's stopping rule~\citep{chernoff1959sequential} \ambuj{description of "track and stop" didn't make much sense to me}.
For the tight lower bound result on the sample complexity, we refer the reader to~\citet{garivier2016optimal}. \ambuj{we could add some actual bounds to this section just to give the reader an idea of what's achievable}





